GW231123: extreme spins or microglitches?

The recently reported binary black hole merger, GW231123, has unusual properties that make it hard to explain astrophysically. Parameter estimation studies are consistent with maximally spinning black holes and the dimensionless spin of the more massive component is constrained to be $\chi_1\gtrsim 0.8$. Analysis of data also revealed potential systematics that could not be fully replicated with simulated studies. We explore the possibility that these measurements are biased due to unmodeled non-Gaussian noise in the detectors, and that the actual black hole spins are more modest. We present evidence for a population of \textit{microglitches} in LIGO gravitational-wave strain data that can lead to biases in the parameter estimation of short-duration signals such as GW231123. Using simulated data of a massive event like GW231123, we demonstrate how microglitches can bias our measurements of black hole spins toward $\chi\approx1$ with negligible posterior support for the true value of $\chi\approx0.7$. We develop a noise model to account for microglitches and show that this model successfully reduces biases in the recovery of signal parameters. We characterize the microglitch population in real interferometer data surrounding GW231123 and find a single detector glitch duty cycle of $0.57_{-0.19}^{+0.21}$, which implies nearly a $100\%$ probability that at least one event through the fourth gravitational wave transient catalog coincides with microglitches in two detectors. We argue that further investigations are required before we can have a confident picture of the astrophysical properties of GW231123.

==> macros.tex <==
\newcommand{\redtext}[1]{{\color{red} #1}}
\newcommand{\redcite}[1]{\redtext{(cite #1) }}

\newcommand{\SB}[1]{{\color{blue} (SB: #1)}}

\newcommand{\SPA}{School of Physics and Astronomy, Monash University, Clayton VIC 3800, Australia}
\newcommand{\OzGravMonash}{OzGrav: The ARC Centre of Excellence for Gravitational Wave Discovery, Clayton VIC 3800, Australia}

